Zero-shot CAD Program Re-Parameterization for Interactive Manipulation

Parametric CAD models encode entire families of shapes that should, in principle, be easy for designers to explore. However, in practice, parametric CAD models can be difficult to manipulate due to implicit semantic constraints among parameter values. Finding and enforcing these semantic constraints solely from geometry or programmatic shape representations is not possible because these constraints ultimately reflect design intent. They are informed by the designer's experience and semantics in the real world. To address this challenge, we introduce a zero-shot pipeline that leverages pre-trained large language and image model to infer meaningful space of variations for a shape. We then re-parameterize a new constrained parametric CAD program that captures these variations, enabling effortless exploration of the design space along meaningful design axes.

==> ccs.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010371.10010396.10010399</concept_id>
       <concept_desc>Computing methodologies~Parametric curve and surface models</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010148.10010149</concept_id>
       <concept_desc>Computing methodologies~Symbolic and algebraic algorithms</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10003752.10003766.10003767.10003769</concept_id>
       <concept_desc>Theory of computation~Rewrite systems</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Parametric curve and surface models}
\ccsdesc[300]{Computing methodologies~Symbolic and algebraic algorithms}
\ccsdesc[500]{Theory of computation~Rewrite systems}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{parametric modeling, program synthesis}

==> sec/7_figures.tex <==
\clearpage

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{img/generation-gallery.pdf}
    \caption{A gallery of text-condition CAD parameter optimization of different input models (first column) towards varying prompts.}
    \label{fig:generation-gallery}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{img/ablation-multiple-sd.pdf}
    \caption{Rendered and diffusion-generated images at different iterations during optimization using (top) one diffusion-generated image per camera pose; (middle) three images; and (bottom) three images and select one image that is closest to the rendering. Note that the camera angles for the diffusion-generated images are random.}
    \label{fig:ablation-num-sd}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{img/constrained-gallery-2.pdf}
    \caption{A gallery of design variations using the constrained inferred from our pipeline.}
    \label{fig:constraint-gallery}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{img/constrained-gallery.pdf}
    \caption{(a) Imperfections on interpolated results without the constraints. (b) Generation results using different loss functions: CLIP similarity, distillation score, L2 difference of the image latent of the rendered and diffusion-generated images, and L2 difference in the images (c) A gallery of chairs when all constraints of the base model are imposed. (d) Peculiar shape of generated ``rocking chair'' and ``dining table'' (left) and the image guidance (right).}
    \label{fig:misc}
\end{figure*}

    % \caption{}
